Sample-Efficient Algorithms for Recovering Structured Signals from Magnitude-Only Measurements

We consider the problem of recovering a signal $\mathbf{x}^* \in \mathbf{R}^n$, from magnitude-only measurements $y_i = |\left\langle\mathbf{a}_i,\mathbf{x}^*\right\rangle|$ for $i=[m]$. Also called the phase retrieval, this is a fundamental challenge in bio-,astronomical imaging and speech processing. The problem above is ill-posed; additional assumptions on the signal and/or the measurements are necessary. In this paper we first study the case where the signal $\mathbf{x}^*$ is $s$-sparse. We develop a novel algorithm that we call Compressive Phase Retrieval with Alternating Minimization, or CoPRAM. Our algorithm is simple; it combines the classical alternating minimization approach for phase retrieval with the CoSaMP algorithm for sparse recovery. Despite its simplicity, we prove that CoPRAM achieves a sample complexity of $O(s^2\log n)$ with Gaussian measurements $\mathbf{a}_i$, matching the best known existing results; moreover, it demonstrates linear convergence in theory and practice. Additionally, it requires no extra tuning parameters other than signal sparsity $s$ and is robust to noise. When the sorted coefficients of the sparse signal exhibit a power law decay, we show that CoPRAM achieves a sample complexity of $O(s\log n)$, which is close to the information-theoretic limit. We also consider the case where the signal $\mathbf{x}^*$ arises from structured sparsity models. We specifically examine the case of block-sparse signals with uniform block size of $b$ and block sparsity $k=s/b$. For this problem, we design a recovery algorithm Block CoPRAM that further reduces the sample complexity to $O(ks\log n)$. For sufficiently large block lengths of $b=\Theta(s)$, this bound equates to $O(s\log n)$. To our knowledge, this constitutes the first end-to-end algorithm for phase retrieval where the Gaussian sample complexity has a sub-quadratic dependence on the signal sparsity level.

==> results/noise_effect.tex <==
\begin{tikzpicture}
\begin{axis}
[width=0.4\textwidth,
xlabel= Noise-to-signal ratio NSR, 
ylabel= Relative error in recovery,
grid style = dashed,
grid=both,
legend style={at={(1.8,0.3)}, anchor=south east, %legend columns=-1,
} 
]


\addplot[color=blue,mark=square*] plot coordinates {
	(0.1,     0.0861)
	(0.2,     0.1478)
	(0.3,     0.1949)
	(0.4,     0.2764)
	(0.5,     0.3533)
	(0.6,     0.5516)
	(0.7,     0.6584)
	(0.8,     0.8303)
	(0.9,     0.9044)
	(1,       0.9854)
};
\addlegendentry{CoPRAM};

\addplot plot coordinates {
	(0.1,     0.0432)
	(0.2,     0.0649)
	(0.3,     0.1001)
	(0.4,     0.1074)
	(0.5,     0.1697)
	(0.6,     0.2718)
	(0.7,     0.3557)
	(0.8,     0.4534)
	(0.9,     0.4720)
	(1,       0.6449)
};
\addlegendentry{Block CoPRAM};

\addplot[color=green,mark=*] plot coordinates {
(0.1,     0.0933)
(0.2,     0.1607)
(0.3,     0.2189)
(0.4,     0.3784)
(0.5,     0.5836)
(0.6,     0.7018)
(0.7,     0.7899)
(0.8,     0.8507)
(0.9,     0.8999)
(1,       0.9076)
};
\addlegendentry{SPARTA};

\end{axis}
\end{tikzpicture}

==> results/transition_graphs_20.tex <==
\begin{tikzpicture}
\begin{axis}
[width=0.4\textwidth,
xlabel= Number of samples $m$, 
ylabel= Probability of recovery,
grid style = dashed,
grid=both,
legend style=
{
%at={(1.6,0.56), %for arxiv version
at={(1.65,0.8),  %for NIPS version
anchor=south west},
cells={align=center}, 
%legend columns=-1,
} 
]

\addplot[color=blue,mark=square*] plot coordinates {
	(200,     0)
	(400,    0.12)
	(600,    0.74)
	(800,    0.94)
	(1000,   1)
	(1200,   1)
	(1400,   1)
	(1600,   1)
	(1800,   1)
	(2000,   1)
};
\addlegendentry{CoPRAM};

\addplot plot coordinates {
(200,    0.14)
(400,    0.58)
(600,    0.98)
(800,    1)
(1000,   1)
(1200,   1)
(1400,   1)
(1600,   1)
(1800,   1)
(2000,   1)
};

\addlegendentry{Block \\CoPRAM};

\addplot plot coordinates {
(200,     0)
(400,     0)
(600,     0)
(800,     0.06)
(1000,    0.58)
(1200,    0.7)
(1400,    0.9)
(1600,    1)
(1800,    1)
(2000,    1)
};
\addlegendentry{ThWF};

\addplot[color=green,mark=*] plot coordinates {
(200,     0)
(400,     0.08)
(600,     0.66)
(800,     0.88)
(1000,    0.98)
(1200,    1)
(1400,    1)
(1600,    1)
(1800,    1)
(2000,    1)
};
\addlegendentry{SPARTA};

%\legend{CoPRAM\\Block CoPRAM\\ThWF\\SPARTA\\}

\end{axis}
\end{tikzpicture}

==> results/transition_graphs_30.tex <==
\begin{tikzpicture}
\begin{axis}
[width=0.4\textwidth,
xlabel= Number of samples $m$, 
ylabel= Probability of recovery,
grid style = dashed,
grid=both,
legend style={at={(1.2,1.2)}, anchor=north east, legend columns=-1,
} 
]

\addplot[color=blue,mark=square*] plot coordinates {
	(200,     0)
	(400,     0)
	(600,     0.04)
	(800,     0.34)
	(1000,    0.58)
	(1200,    0.82)
	(1400,    1)
	(1600,    1)
	(1800,    1.0)
	(2000,    1.0)
};

\addplot plot coordinates {
(200,    0.02)
(400,    0.38)
(600,    0.78)
(800,    0.96)
(1000,   1)
(1200,   0.98)
(1400,   1)
(1600,   1)
(1800,   1)
(2000,   1)
};

\addplot plot coordinates {
(200,     0)
(400,     0)
(600,     0)
(800,     0)
(1000,    0.18)
(1200,    0.38)
(1400,    0.7667)
(1600,    0.96)
(1800,    0.9333)
(2000,    0.98)
};

\addplot[color=green,mark=*] plot coordinates {
(200,     0)
(400,     0)
(600,     0.02)
(800,     0.18)
(1000,    0.46)
(1200,    0.74)
(1400,    0.8333)
(1600,    1)
(1800,    0.9667)
(2000,    1)
};

%\legend{$CoPRAM$\\$BCoPRAM$\\$ThWF$\\$SPARTA$\\}

\end{axis}
\end{tikzpicture}
